On the Force-Freeness of the Photospheric Sunspot Magnetic Fields as Observed from Hinode (SOT/SP)

A magnetic field is force-free if there is no interaction between the magnetic field and plasma in surrounding atmosphere i.e., electric currents are aligned with the magnetic field, giving rise to zero Lorentz force. Computation of various magnetic parameters such as magnetic energy, gradient of twist of sunspot fields and any kind of extrapolations, heavily hinge on the force-free approximation of the photospheric sunspot magnetic fields. Thus it is important to inspect the force-freeness of sunspot fields. The force-freeness of sunspot magnetic fields has been examined earlier by some researchers ending with incoherent results. Accurate photospheric vector field measurements with high spatial resolution are required to inspect the force-free nature of sunspots. We use several such vector magnetograms obtained from the Solar Optical Telescope/Spectro-Polarimeter aboard the Hinode. Both necessary and sufficient conditions for force-freeness are examined by checking global and local nature of magnetic forces over sunspots. We find that the sunspot magnetic fields are not much away from force-free configuration, although they are not completely force-free on the photosphere. The umbral and inner penumbral fields are more force-free than the middle and the outer penumbral fields. During their evolution, sunspot magnetic fields are found to maintain their proximity to force-free behaviour. Although a dependence of net Lorentz force components is seen on the evolutionary stages of the sunspots, we don't find a systematic relationship between the nature of sunspot fields and associated flare activity. Further, we examine whether the fields at photosphere follow linear or non-linear force free conditions. After examining this in various complex and simple sunspots we conclude that,in either case,the photospheric sunspot fields are closer to satisfy non linear force-free field approximation.

==> journ_abbre.tex <==
%RR ## to be adapted when the volume number is known
\def\thisvolume{these proceedings}

%RR journal abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aj{{AJ}}			
\def\araa{{ARA\&A}}		
\def\apj{{ApJ}}			
\def\apjl{{ApJ}}		
\def\apjs{{ApJS}}		
\def\ao{{Appl.\ Optics}}
\def\apss{{Ap\&SS}}		
\def\aap{{A\&A}}		
\def\aapr{{A\&A~Rev.}}		
\def\aaps{{A\&AS}}		
\def\an{{Astron.\ Nachrichten}}
\def\aspcs{{ASP Conf.\ Ser.}}
\def\azh{{AZh}}			
\def\baas{{BAAS}}		
\def\grl{{Geophysics Research Letters}}
\def\jgr{{Journal of Geophysical Research}}
\def\jrasc{{JRASC}}		
\def\memras{{MmRAS}}		
\def\mnras{{MNRAS}}
\def\nat{{Nature}}		
\def\pra{{Phys.\ Rev.\ A}}
\def\prb{{Phys.\ Rev.\ B}}		
\def\prc{{Phys.\ Rev.\ C}}		
\def\prd{{Phys.\ Rev.\ D}}		
\def\prl{{Phys.\ Rev.\ Lett}}	
\def\pasp{{PASP}}
\def\pasj{{PASJ}}		
\def\qjras{{QJRAS}}
\def\science{{Science}}		
\def\skytel{{S\&T}}		
\def\solphys{{Solar\ Phys.}}
\def\sovast{{Soviet\ Ast.}}
\def\ssr{{Space\ Sci.\ Rev.}}
\def\svassp{{Astrophys.\ Space Science Proc.}}
\def\zap{{ZAp}}			
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs

%%%;;;;;;;more-added:sanjiv;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
%\verb"\araa" & Annual Review of Astronomy and Astrophysics\\
%\verb"\actaa" & Acta Astronomica\\
%\verb"\ao" & Applied Optics\\
%\verb"\aj" & Astronomical Journal\\
%\verb"\azh" & Astronomicheskii Zhurnal\\
%\verb"\aap" & Astronomy and Astrophysics\\
%\verb"\aapr" & Astronomy and Astrophysics Reviews\\
%\verb"\apj" & Astrophysical Journal\\
%\verb"\apjl" & \rule[.5ex]{2em}{.4pt}, Letters to the Editor\\
%\verb"\apjs" & \rule[.5ex]{2em}{.4pt}, Supplement Series\\
%\verb"\aplett" & Astrophysics Letters and Communications\\
%\verb"\apspr" & Astrophysics Space Physics Research\\
%\verb"\apss" & Astrophysics and Space Science\\
%\verb"\aaps" & \rule[.5ex]{2em}{.4pt}, Supplement Series\\
%\verb"\baas" & Bulletin of the AAS\\
%\verb"\bain" & Bulletin Astronomical Inst. Netherlands\\
%\verb"\caa" & Chinese Astronomy and Astrophysics\\
%\verb"\cjaa" & Chinese Journal of Astronomy and Astrophysics\\
%\verb"\fcp" & Fundamental Cosmic Physics\\
%\verb"\gca" & Geochimica Cosmochimica Acta\\
%\verb"\grl" & Geophysics Research Letters\\
%\verb"\iaucirc" & IAU Circular\\
%\verb"\icarus" & Icarus\\
%\verb"\jcp" & Journal of Chemical Physics\\
%\verb"\jgr" & Journal of Geophysical Research\\
%\verb"\jcap" & Journal of Cosmology and Astroparticle Physics\\
%\verb"\jqsrt" & Journal of Quantitative Specstroscopy and Radiative Transfer\\
%\verb"\jrasc" & Journal of the RAS of Canada\\
%\verb"\memras" & Memoirs of the RAS\\
%\verb"\memsai" & Mem. Societa Astronomica Italiana\\
%\verb"\mnras" & Monthly Notices of the RAS\\
%\verb"\na" & New Astronomy\\
%\verb"\nar" & New Astronomy Review\\
%\verb"\nat" & Nature\\
%\verb"\nphysa" & Nuclear Physics A\\
%\verb"\physscr" & Physica Scripta\\
%\verb"\pra" & Physical Review A\\
%\verb"\prb" & Physical Review B\\
%\verb"\prc" & Physical Review C\\
%\verb"\prd" & Physical Review D\\
%\verb"\pre" & Physical Review E\\
%\verb"\prl" & Physical Review Letters\\
%\verb"\physrep" & Physics Reports\\
%\verb"\planss" & Planetary Space Science\\
%\verb"\procspie" & Proceedings of the SPIE\\
%\verb"\pasa" & Publications of the ASA\\
%\verb"\pasj" & Publications of the ASJ\\
%\verb"\pasp" & Publications of the ASP\\
%\verb"\qjras" & Quarterly Journal of the RAS\\
%\verb"\rmxaa" & Revista Mexicana de Astronomia y Astrofisica \\
%\verb"\skytel" & Sky and Telescope\\
%\verb"\solphys" & Solar Physics\\
%\verb"\ssr" & Space Science Reviews\\
%%%;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;

%RR astronomy and math commands copied from ASP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ion#1#2{{\rm #1}\,{\uppercase{#2}}}  %RR ~>\, \sc > uc
\def\deg{\hbox{$^\circ$}}
\def\sun{\hbox{$\odot$}}
\def\earth{\hbox{$\oplus$}}
\def\la{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\ga{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\def\sq{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\arcmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\fd{\hbox{$.\!\!^{\rm d}$}}
\def\fh{\hbox{$.\!\!^{\rm h}$}}
\def\fm{\hbox{$.\!\!^{\rm m}$}}
\def\fs{\hbox{$.\!\!^{\rm s}$}}
\def\fdg{\hbox{$.\!\!^\circ$}}
\def\farcm{\hbox{$.\mkern-4mu^\prime$}}
\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}
\def\fp{\hbox{$.\!\!^{\scriptscriptstyle\rm p}$}}
\def\micron{\hbox{$\mu$m}}
\def\onehalf{\hbox{$\,^1\!/_2$}}	
\def\onethird{\hbox{$\,^1\!/_3$}}
\def\twothirds{\hbox{$\,^2\!/_3$}}
\def\onequarter{\hbox{$\,^1\!/_4$}}
\def\threequarters{\hbox{$\,^3\!/_4$}}
\def\ubv{\hbox{$U\!BV$}}		
\def\ubvr{\hbox{$U\!BV\!R$}}		
\def\ubvri{\hbox{$U\!BV\!RI$}}		
\def\ubvrij{\hbox{$U\!BV\!RI\!J$}}		
\def\ubvrijh{\hbox{$U\!BV\!RI\!J\!H$}}		
\def\ubvrijhk{\hbox{$U\!BV\!RI\!J\!H\!K$}}		
\def\ub{\hbox{$U\!-\!B$}}		
\def\bv{\hbox{$B\!-\!V$}}		
\def\vr{\hbox{$V\!-\!R$}}		
\def\ur{\hbox{$U\!-\!R$}}		


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%RR RJR additional commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%RR -- non-bullet item marker in itemize list
\def\labelitemi{{\bf --}}

%RR -- latin abbreviations
\def\rmit#1{{\it #1}}              %% italics (RR style, Kluwer)
\def\rmit#1{{\rm #1}}              %% redefine for ASP, A&A, ApJ, Springer??
\def\etal{\rmit{et al.}}           %% use \etal\ for space behind it
\def\etc{\rmit{etc.}}
\def\ie{\rmit{i.e.,}}              %% , required (Webster 1681)
\def\eg{\rmit{e.g.,}}              %% , required (Webster 1681)
\def\cf{cf.}                       %% no Latin, always Roman (Webster 1686)
\def\viz{\rmit{viz.}}
\def\vs{\rmit{vs.}}

%RR -- mathematical
\def\rot{\hbox{\rm rot}}
\def\div{\hbox{\rm div}}
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\def\dif{\: {\rm d}}                       %% differential d with space
\def\ep{\:{\rm e}^}                        %% e^ with space and roman e
\def\dash{\hbox{$\,-\,$}}                  %% math-like hyphen
\def\is{\!=\!}                             %% = in text for tighter spacing

%RR --stellar stuff
\def\starname#1#2{${#1}$\,{\rm {#2}}}  %% \starname{\alpha}{Cen~A}
\def\Teff{\hbox{$T_{\rm eff}$}}

%RR -- units (in addition to the ASP ones above)
\def\kms{\hbox{km$\;$s$^{-1}$}}
\def\Mxcm{\hbox{Mx\,cm$^{-2}$}}    %% no 2, damn tex

%RR -- magnetic field
\def\Bapp{\hbox{$B_{\rm app}$}}    %% apparent flux density, Lites convention

%RR -- oscillations
\def\komega{($k, \omega$)}                 %% k - omega
\def\kf{($k_h,f$)}                         %% f - k_h
\def\VminI{\hbox{$V\!\!-\!\!I$}}           %% V-I
\def\IminI{\hbox{$I\!\!-\!\!I$}}           %% I-I
\def\VminV{\hbox{$V\!\!-\!\!V$}}           %% V-V
\def\Xt{\hbox{$X\!\!-\!t$}}                %% X-t

%RR -- atomic levels
%%      use:    \level 3s3p 3Pe
%%              \level 3s$^2$ {1,3}P{e,o}
%%              \level {} 3Ge
\def\level #1 #2#3#4{$#1 \: ^{#2} \mbox{#3} ^{#4}$}

%RR -- some spectral species
\def\specchar#1{\uppercase{#1}}    %% to be redefined for A&A = \sc
\def\AlI{\mbox{Al\,\specchar{i}}}  %% use \AlI\ for space behind it
\def\BI{\mbox{B\,\specchar{i}}}
\def\BII{\mbox{B\,\specchar{ii}}}
\def\BaI{\mbox{Ba\,\specchar{i}}}
\def\BaII{\mbox{Ba\,\specchar{ii}}}
\def\CI{\mbox{C\,\specchar{i}}}
\def\CII{\mbox{C\,\specchar{ii}}}
\def\CIII{\mbox{C\,\specchar{iii}}}
\def\CIV{\mbox{C\,\specchar{iv}}}
\def\CaI{\mbox{Ca\,\specchar{i}}}
\def\CaII{\mbox{Ca\,\specchar{ii}}}
\def\CaIII{\mbox{Ca\,\specchar{iii}}}
\def\CoI{\mbox{Co\,\specchar{i}}}
\def\CrI{\mbox{Cr\,\specchar{i}}}
\def\CriI{\mbox{Cr\,\specchar{ii}}}
\def\CsI{\mbox{Cs\,\specchar{i}}}
\def\CsII{\mbox{Cs\,\specchar{ii}}}
\def\CuI{\mbox{Cu\,\specchar{i}}}
\def\FeI{\mbox{Fe\,\specchar{i}}}
\def\FeII{\mbox{Fe\,\specchar{ii}}}
\def\FeIX{\mbox{Fe\,\specchar{ix}}}
\def\FeX{\mbox{Fe\,\specchar{x}}}
\def\FeXVI{\mbox{Fe\,\specchar{xvi}}}
\def\FrI{\mbox{Fr\,\specchar{i}}}
\def\HI{\mbox{H\,\specchar{i}}}
\def\HII{\mbox{H\,\specchar{ii}}}
\def\Hmin{\hbox{\rmH$^{^{_{\scriptstyle -}}}$}}      %% H^min, elegant
\def\Hemin{\hbox{{\rm He}$^{^{_{\scriptstyle -}}}$}} %% He^min, idem
\def\HeI{\mbox{He\,\specchar{i}}}
\def\HeII{\mbox{He\,\specchar{ii}}}
\def\HeIII{\mbox{He\,\specchar{iii}}}
\def\KI{\mbox{K\,\specchar{i}}}
\def\KII{\mbox{K\,\specchar{ii}}}
\def\KIII{\mbox{K\,\specchar{iii}}}
\def\LiI{\mbox{Li\,\specchar{i}}}
\def\LiII{\mbox{Li\,\specchar{ii}}}
\def\LiIII{\mbox{Li\,\specchar{iii}}}
\def\MgI{\mbox{Mg\,\specchar{i}}}
\def\MgII{\mbox{Mg\,\specchar{ii}}}
\def\MgIII{\mbox{Mg\,\specchar{iii}}}
\def\MnI{\mbox{Mn\,\specchar{i}}}
\def\NI{\mbox{N\,\specchar{i}}}
\def\NaI{\mbox{Na\,\specchar{i}}}
\def\NaII{\mbox{Na\,\specchar{ii}}}
\def\NaIII{\mbox{Na\,\specchar{iii}}}
\def\NiI{\mbox{Ni\,\specchar{i}}}
\def\NiII{\mbox{Ni\,\specchar{ii}}}
\def\NiIII{\mbox{Ni\,\specchar{iii}}}
\def\OI{\mbox{O\,\specchar{i}}}
\def\OVI{\mbox{O\,\specchar{vi}}}
\def\RbI{\mbox{Rb\,\specchar{i}}}
\def\SII{\mbox{S\,\specchar{ii}}}
\def\SiI{\mbox{Si\,\specchar{i}}}
\def\SiII{\mbox{Si\,\specchar{ii}}}
\def\SrI{\mbox{Sr\,\specchar{i}}}
\def\SrII{\mbox{Sr\,\specchar{ii}}}
\def\TiI{\mbox{Ti\,\specchar{i}}}
\def\TiII{\mbox{Ti\,\specchar{ii}}}
\def\TiIII{\mbox{Ti\,\specchar{iii}}}
\def\TiIV{\mbox{Ti\,\specchar{iv}}}
\def\VI{\mbox{V\,\specchar{i}}}
\def\HtwoO{\mbox{H$_2$O}}        %% H2O %RR TeX doesn't accept numbers alas
\def\Otwo{\mbox{O$_2$}}          %% O2

%RR -- hydrogen spectrum features
\def\Halpha{\mbox{H\hspace{0.1ex}$\alpha$}} %% \Halpha\ for space behind it
\def\Ha{\mbox{H\hspace{0.2ex}$\alpha$}}
\def\Hbeta{\mbox{H\hspace{0.2ex}$\beta$}}
\def\Hgamma{\mbox{H\hspace{0.2ex}$\gamma$}}
\def\Hdelta{\mbox{H\hspace{0.2ex}$\delta$}}
\def\Hepsilon{\mbox{H\hspace{0.2ex}$\epsilon$}}
\def\Hzeta{\mbox{H\hspace{0.2ex}$\zeta$}}
\def\Lyalpha{\mbox{Ly$\hspace{0.2ex}\alpha$}}
\def\Lybeta{\mbox{Ly$\hspace{0.2ex}\beta$}}
\def\Lygamma{\mbox{Ly$\hspace{0.2ex}\gamma$}}
\def\Lycont{\mbox{Ly\hspace{0.2ex}{\small cont}}}
\def\Baalpha{\mbox{Ba$\hspace{0.2ex}\alpha$}}
\def\Babeta{\mbox{Ba$\hspace{0.2ex}\beta$}}
\def\Bacont{\mbox{Ba\hspace{0.2ex}{\small cont}}}
\def\Paalpha{\mbox{Pa$\hspace{0.2ex}\alpha$}}
\def\Bralpha{\mbox{Br$\hspace{0.2ex}\alpha$}}

%RR -- Na D
\def\NaD{\mbox{Na\,\specchar{i}\,D}}    %% use \NaD\ for space behind it
\def\NaDone{\mbox{Na\,\specchar{i}\,\,D$_1$}}
\def\NaDtwo{\mbox{Na\,\specchar{i}\,\,D$_2$}}
\def\NaID{\mbox{Na\,\specchar{i}\,\,D}}
\def\NaIDone{\mbox{Na\,\specchar{i}\,\,D$_1$}}
\def\NaIDtwo{\mbox{Na\,\specchar{i}\,\,D$_2$}}
\def\Done{\mbox{D$_1$}}
\def\Dtwo{\mbox{D$_2$}}

%RR -- Mg b
\def\Mgbone{\mbox{Mg\,\specchar{i}\,b$_1$}}
\def\Mgbtwo{\mbox{Mg\,\specchar{i}\,b$_2$}}
\def\Mgbthree{\mbox{Mg\,\specchar{i}\,b$_3$}}
\def\MgIb{\mbox{Mg\,\specchar{i}\,b}}
\def\MgIbone{\mbox{Mg\,\specchar{i}\,b$_1$}}
\def\MgIbtwo{\mbox{Mg\,\specchar{i}\,b$_2$}}
\def\MgIbthree{\mbox{Mg\,\specchar{i}\,b$_3$}}

%RR -- Ca II H & K
\def\CaIIK{\mbox{Ca\,\specchar{ii}\,K}}       %% use \CaIIK\ for space
\def\CaIIH{\mbox{Ca\,\specchar{ii}\,H}}
\def\CaIIHK{\mbox{Ca\,\specchar{ii}\,H\,\&\,K}}
\def\HK{\mbox{H\,\&\,K}}
\def\Kthree{\mbox{K$_3$}}      %% numbers not permitted, alas
\def\Hthree{\mbox{H$_3$}}
\def\Ktwo{\mbox{K$_2$}}
\def\Htwo{\mbox{H$_2$}}
\def\Kone{\mbox{K$_1$}}
\def\Hone{\mbox{H$_1$}}
\def\KtwoV{\mbox{K$_{2V}$}}
\def\KtwoR{\mbox{K$_{2R}$}}
\def\KoneV{\mbox{K$_{1V}$}}
\def\KoneR{\mbox{K$_{1R}$}}
\def\HtwoV{\mbox{H$_{2V}$}}
\def\HtwoR{\mbox{H$_{2R}$}}
\def\HoneV{\mbox{H$_{1V}$}}
\def\HoneR{\mbox{H$_{1R}$}}

%RR -- Mg II h & k
\def\hk{\mbox{h\,\&\,k}}
\def\kthree{\mbox{k$_3$}}
\def\hthree{\mbox{h$_3$}}
\def\ktwo{\mbox{k$_2$}}
\def\htwo{\mbox{h$_2$}}
\def\kone{\mbox{k$_1$}}
\def\hone{\mbox{h$_1$}}
\def\ktwoV{\mbox{k$_{2V}$}}
\def\ktwoR{\mbox{k$_{2R}$}}
\def\koneV{\mbox{k$_{1V}$}}
\def\koneR{\mbox{k$_{1R}$}}
\def\htwoV{\mbox{h$_{2V}$}}
\def\htwoR{\mbox{h$_{2R}$}}
\def\honeV{\mbox{h$_{1V}$}}
\def\honeR{\mbox{h$_{1R}$}}

